First Order Locally Orderless Registration

First Order Locally Orderless Registration (FLOR) is a scale-space framework for image density estimation used for defining image similarity, mainly for Image Registration. The Locally Orderless Registration framework was designed in principle to use zeroth-order information, providing image density estimates over three scales: image scale, intensity scale, and integration scale. We extend it to take first-order information into account and hint at higher-order information. We show how standard similarity measures extend into the framework. We study especially Sum of Squared Differences (SSD) and Normalized Cross-Correlation (NCC) but present the theory of how Normalised Mutual Information (NMI) can be included.

==> authors.tex <==
\author{José D. Tascón-Vidarte\inst{1}\orcidID{0000-1111-2222-3333} \and
Kenny Erleben\inst{1}\orcidID{0000-1111-2222-3333} \and
%Jose tascon\inst{1}\orcidID{0000-1111-2222-3333} \and
Francois Lauze\inst{2,3}\orcidID{1111-2222-3333-4444} \and
Sune Darkner\inst{3}\orcidID{2222--3333-4444-5555}}
%
\authorrunning{F. Author et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%
\institute{University of copenhagen 
\email{darkner@di.ku.dk}\\
}
%


==> custom_settings.tex <==
\usepackage{blindtext}

\usepackage{amsmath}
\usepackage{francois-preamble}
\usepackage{graphicx,cleveref}

% Used for displaying a sample figure. If possible, figure files should
% be included in EPS format.
%
% If you use the hyperref package, please uncomment the following line
% to display URLs in blue roman font according to Springer's eBook style:
% \renewcommand\UrlFont{\color{blue}\rmfamily}


\usepackage[ruled]{algorithm2e} % For algorithms
\renewcommand{\algorithmcfname}{ALGORITHM}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}


%\newcommand{\abs}[1]{\left| {#1} \right|}
%\newcommand{\acos }{ \ensuremath{ \cos^{-1} } }
%\newcommand{\asin }{ \ensuremath{ \sin^{-1} } }
%\newcommand{\atan }{ \ensuremath{ \phantom{\cdot}\text{atan}_2 } }
%\newcommand{\ball}{\ensuremath{ \mathcal{B} }}
%\newcommand{\bigO}{ \ensuremath{ \mathcal{O} }}
%\newcommand{\degree}{\,^{\circ}}
%\renewcommand{\det}[1]{ \ensuremath{ \text{det}\left( #1 \right) } }
%\newcommand{\hull }[1]{ \ensuremath{ \text{convex hull}\left( #1 \right) } }
%\newcommand{\identity}{ \ensuremath{ \mat I }}
%\newcommand{\idx }[1]{ \ensuremath{ \mathbb{#1} } }
%\newcommand{\intersection}{\ensuremath{ \cap }}
%\newcommand{\logand }{ \ensuremath{ \wedge } }
%\newcommand{\logor }{ \ensuremath{ \vee } }
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1} }}
%\newcommand{\interior}[1]{\ensuremath{ {#1}^{\circ} }}
%\newcommand{\boundary}[1]{\ensuremath{ \partial{#1} }}
%\newcommand{\N}{ \mathbb{N} }
\newcommand{\norm}[1]{\parallel {#1} \parallel}
%\newcommand{\proj }[1]{ \ensuremath{ \text{proj}\left( #1 \right) } }
%\newcommand{\prox }[2]{ \ensuremath{ \text{prox}_{#1}\left( #2 \right) } }
%\newcommand{\quat}[1]{ #1 }
\renewcommand{\Re}{ \mathbb{R} }
\newcommand{\Z}{ \mathbb{Z} }
\newcommand{\set}[1]{\mathcal{#1}}
%\newcommand{\seq}[1]{ \left\{ #1 \right\} }
%\newcommand{\sgn }[1]{ \ensuremath{ \text{sgn}\left( #1 \right) } }
%\newcommand{\smallO}{\ensuremath{ \mathbf{o} }}
\renewcommand{\th}{ \ensuremath{ ^{\text{th}}} }
%\newcommand{\trace }[1]{ \ensuremath{ \text{tr}\left( #1 \right) } }
%\newcommand{\union}{\ensuremath{ \cup }}
%\renewcommand{\vec}[1]{ \ensuremath{\mathbf{#1} } }
%\newcommand{\activeset}{ \mathcal{ A } }
%\newcommand{\allset}{ \mathcal{ E } \cup \mathcal{I} }
%\newcommand{\arctantwo}{\ensuremath{\arctan\!2}}
%\newcommand{\crossmat}[1]{\ensuremath{\boldsymbol{#1}^{\times} }}
%\newcommand{\curl}{\operatorname{\text{curl}}}
%\newcommand{\diag}{\operatorname{\text{diag}}}
%\newcommand{\divergence}{\operatorname{\text{div}}}
%\newcommand{\enorm}[1]{\ensuremath{\left\| #1 \right\|_{_2}}}
%\newcommand{\equalityset}{ \mathcal{ E } }
%\newcommand{\feasibledirections}{ \ensuremath{\mathcal{F}} }
%\newcommand{\feasibleregion}{ \ensuremath{\Omega} }
%\newcommand{\func}[1]{{\bf{#1}}}
%\newcommand{\grad}{\operatorname{\nabla}}
%\newcommand{\inequalityset}{ \mathcal{ I } }
%\newcommand{\jacobian}[1]{\ensuremath{\boldsymbol{\mathit{#1}} }}
%\newcommand{\lagrangian}{ \mathcal{ L } }
%\newcommand{\rtm}{$^{\textrm{®}}$} % Registred trademark  \textregistered
%\newcommand{\tangentcone}{ \ensuremath{ \mathcal{ T }_{\Omega} } }
%\newcommand{\vecop}{\operatorname{\text{vec}}}
%\newcommand{\FG}{ \mathcal{G} }
%\newcommand{\FC}{ \mathcal{F} }
%\newcommand{\LS}{ \mathcal{L} }


\newcommand{\sdf}{ \phi }
\newcommand{\A}{ \mathtt{A} }
\newcommand{\B}{ \mathtt{B} }
\newcommand{\CA}{ \mathtt{C} }
\newcommand{\faces}{ \mathcal{F} }
\newcommand{\tetrahedra}{ \mathcal{T} }
\newcommand{\vertices}{ \mathcal{V} }
\newcommand{\indices}{ \mathcal{I} }

\newcommand{\conv}{ * }
\newcommand{\lift}{ \hat{\conv} }



\usepackage{color} 
\definecolor{color1}{rgb}{0.5,0.1,0.1}
\definecolor{color2}{rgb}{0.1,0.5,0.1}
\definecolor{color3}{rgb}{0.1,0.1,0.5}
\definecolor{color4}{rgb}{0.5,0.1,0.5}
\newcommand{\kenny}[1]{{ \color{color1} K: #1}}

